Continuum modelling and simulation of granular flows through their many phases

We propose and numerically implement a constitutive framework for granular media that allows the material to traverse through its many common phases during the flow process. When dense, the material is treated as a pressure sensitive elasto-viscoplastic solid obeying a yield criterion and a plastic flow rule given by the $\mu(I)$ inertial rheology of granular materials. When the free volume exceeds a critical level, the material is deemed to separate and is treated as disconnected, stress-free media. A Material Point Method (MPM) procedure is written for the simulation of this model and many demonstrations are provided in different geometries. By using the MPM framework, extremely large strains and nonlinear deformations, which are common in granular flows, are representable. The method is verified numerically and its physical predictions are validated against known results.

==> python-generated-grids.tex <==

\node[inactivempmnode] (GNi0j0) at ($(0.000000in,0.000000in) + (CS1)$) {};
\node[inactivempmnode] (GNi0j1) at ($(0.000000in,0.325000in) + (CS1)$) {};
\node[inactivempmnode] (GNi0j2) at ($(0.000000in,0.650000in) + (CS1)$) {};
\node[inactivempmnode] (GNi0j3) at ($(0.000000in,0.975000in) + (CS1)$) {};
\node[inactivempmnode] (GNi0j4) at ($(0.000000in,1.300000in) + (CS1)$) {};
\node[inactivempmnode] (GNi1j0) at ($(0.325000in,0.000000in) + (CS1)$) {};
\node[inactivempmnode] (GNi1j1) at ($(0.325000in,0.325000in) + (CS1)$) {};
\node[inactivempmnode] (GNi1j2) at ($(0.325000in,0.650000in) + (CS1)$) {};
\node[inactivempmnode] (GNi1j3) at ($(0.325000in,0.975000in) + (CS1)$) {};
\node[inactivempmnode] (GNi1j4) at ($(0.325000in,1.300000in) + (CS1)$) {};
\node[inactivempmnode] (GNi2j0) at ($(0.650000in,0.000000in) + (CS1)$) {};
\node[inactivempmnode] (GNi2j1) at ($(0.650000in,0.325000in) + (CS1)$) {};
\node[inactivempmnode] (GNi2j2) at ($(0.650000in,0.650000in) + (CS1)$) {};
\node[inactivempmnode] (GNi2j3) at ($(0.650000in,0.975000in) + (CS1)$) {};
\node[inactivempmnode] (GNi2j4) at ($(0.650000in,1.300000in) + (CS1)$) {};
\node[inactivempmnode] (GNi3j0) at ($(0.975000in,0.000000in) + (CS1)$) {};
\node[inactivempmnode] (GNi3j1) at ($(0.975000in,0.325000in) + (CS1)$) {};
\node[inactivempmnode] (GNi3j2) at ($(0.975000in,0.650000in) + (CS1)$) {};
\node[inactivempmnode] (GNi3j3) at ($(0.975000in,0.975000in) + (CS1)$) {};
\node[inactivempmnode] (GNi3j4) at ($(0.975000in,1.300000in) + (CS1)$) {};
\node[inactivempmnode] (GNi4j0) at ($(1.300000in,0.000000in) + (CS1)$) {};
\node[inactivempmnode] (GNi4j1) at ($(1.300000in,0.325000in) + (CS1)$) {};
\node[inactivempmnode] (GNi4j2) at ($(1.300000in,0.650000in) + (CS1)$) {};
\node[inactivempmnode] (GNi4j3) at ($(1.300000in,0.975000in) + (CS1)$) {};
\node[inactivempmnode] (GNi4j4) at ($(1.300000in,1.300000in) + (CS1)$) {};
\draw[inactivempmgrid] (GNi0j0) -- (GNi1j0);
\draw[inactivempmgrid] (GNi0j0) -- (GNi0j1);
\draw[inactivempmgrid] (GNi0j1) -- (GNi1j1);
\draw[inactivempmgrid] (GNi0j1) -- (GNi0j2);
\draw[inactivempmgrid] (GNi0j2) -- (GNi1j2);
\draw[inactivempmgrid] (GNi0j2) -- (GNi0j3);
\draw[inactivempmgrid] (GNi0j3) -- (GNi1j3);
\draw[inactivempmgrid] (GNi0j3) -- (GNi0j4);
\draw[inactivempmgrid] (GNi0j4) -- (GNi1j4);
\draw[inactivempmgrid] (GNi1j0) -- (GNi2j0);
\draw[inactivempmgrid] (GNi1j0) -- (GNi1j1);
\draw[inactivempmgrid] (GNi1j1) -- (GNi2j1);
\draw[inactivempmgrid] (GNi1j1) -- (GNi1j2);
\draw[inactivempmgrid] (GNi1j2) -- (GNi2j2);
\draw[inactivempmgrid] (GNi1j2) -- (GNi1j3);
\draw[inactivempmgrid] (GNi1j3) -- (GNi2j3);
\draw[inactivempmgrid] (GNi1j3) -- (GNi1j4);
\draw[inactivempmgrid] (GNi1j4) -- (GNi2j4);
\draw[inactivempmgrid] (GNi2j0) -- (GNi3j0);
\draw[inactivempmgrid] (GNi2j0) -- (GNi2j1);
\draw[inactivempmgrid] (GNi2j1) -- (GNi3j1);
\draw[inactivempmgrid] (GNi2j1) -- (GNi2j2);
\draw[inactivempmgrid] (GNi2j2) -- (GNi3j2);
\draw[inactivempmgrid] (GNi2j2) -- (GNi2j3);
\draw[inactivempmgrid] (GNi2j3) -- (GNi3j3);
\draw[inactivempmgrid] (GNi2j3) -- (GNi2j4);
\draw[inactivempmgrid] (GNi2j4) -- (GNi3j4);
\draw[inactivempmgrid] (GNi3j0) -- (GNi4j0);
\draw[inactivempmgrid] (GNi3j0) -- (GNi3j1);
\draw[inactivempmgrid] (GNi3j1) -- (GNi4j1);
\draw[inactivempmgrid] (GNi3j1) -- (GNi3j2);
\draw[inactivempmgrid] (GNi3j2) -- (GNi4j2);
\draw[inactivempmgrid] (GNi3j2) -- (GNi3j3);
\draw[inactivempmgrid] (GNi3j3) -- (GNi4j3);
\draw[inactivempmgrid] (GNi3j3) -- (GNi3j4);
\draw[inactivempmgrid] (GNi3j4) -- (GNi4j4);
\draw[inactivempmgrid] (GNi4j0) -- (GNi4j1);
\draw[inactivempmgrid] (GNi4j1) -- (GNi4j2);
\draw[inactivempmgrid] (GNi4j2) -- (GNi4j3);
\draw[inactivempmgrid] (GNi4j3) -- (GNi4j4);
\node[activempmnode] (GNi0j0) at ($(0.000000in,0.000000in) + (CS2)$) {};
\node[activempmnode] (GNi0j1) at ($(0.000000in,0.325000in) + (CS2)$) {};
\node[activempmnode] (GNi0j2) at ($(0.000000in,0.650000in) + (CS2)$) {};
\node[activempmnode] (GNi0j3) at ($(0.000000in,0.975000in) + (CS2)$) {};
\node[activempmnode] (GNi0j4) at ($(0.000000in,1.300000in) + (CS2)$) {};
\node[activempmnode] (GNi1j0) at ($(0.325000in,0.000000in) + (CS2)$) {};
\node[activempmnode] (GNi1j1) at ($(0.325000in,0.325000in) + (CS2)$) {};
\node[activempmnode] (GNi1j2) at ($(0.325000in,0.650000in) + (CS2)$) {};
\node[activempmnode] (GNi1j3) at ($(0.325000in,0.975000in) + (CS2)$) {};
\node[activempmnode] (GNi1j4) at ($(0.325000in,1.300000in) + (CS2)$) {};
\node[activempmnode] (GNi2j0) at ($(0.650000in,0.000000in) + (CS2)$) {};
\node[activempmnode] (GNi2j1) at ($(0.650000in,0.325000in) + (CS2)$) {};
\node[activempmnode] (GNi2j2) at ($(0.650000in,0.650000in) + (CS2)$) {};
\node[activempmnode] (GNi2j3) at ($(0.650000in,0.975000in) + (CS2)$) {};
\node[activempmnode] (GNi2j4) at ($(0.650000in,1.300000in) + (CS2)$) {};
\node[activempmnode] (GNi3j0) at ($(0.975000in,0.000000in) + (CS2)$) {};
\node[activempmnode] (GNi3j1) at ($(0.975000in,0.325000in) + (CS2)$) {};
\node[activempmnode] (GNi3j2) at ($(0.975000in,0.650000in) + (CS2)$) {};
\node[activempmnode] (GNi3j3) at ($(0.975000in,0.975000in) + (CS2)$) {};
\node[activempmnode] (GNi3j4) at ($(0.975000in,1.300000in) + (CS2)$) {};
\node[activempmnode] (GNi4j0) at ($(1.300000in,0.000000in) + (CS2)$) {};
\node[activempmnode] (GNi4j1) at ($(1.300000in,0.325000in) + (CS2)$) {};
\node[activempmnode] (GNi4j2) at ($(1.300000in,0.650000in) + (CS2)$) {};
\node[activempmnode] (GNi4j3) at ($(1.300000in,0.975000in) + (CS2)$) {};
\node[activempmnode] (GNi4j4) at ($(1.300000in,1.300000in) + (CS2)$) {};
\draw[activempmgrid] (GNi0j0) -- (GNi1j0);
\draw[activempmgrid] (GNi0j0) -- (GNi0j1);
\draw[activempmgrid] (GNi0j1) -- (GNi1j1);
\draw[activempmgrid] (GNi0j1) -- (GNi0j2);
\draw[activempmgrid] (GNi0j2) -- (GNi1j2);
\draw[activempmgrid] (GNi0j2) -- (GNi0j3);
\draw[activempmgrid] (GNi0j3) -- (GNi1j3);
\draw[activempmgrid] (GNi0j3) -- (GNi0j4);
\draw[activempmgrid] (GNi0j4) -- (GNi1j4);
\draw[activempmgrid] (GNi1j0) -- (GNi2j0);
\draw[activempmgrid] (GNi1j0) -- (GNi1j1);
\draw[activempmgrid] (GNi1j1) -- (GNi2j1);
\draw[activempmgrid] (GNi1j1) -- (GNi1j2);
\draw[activempmgrid] (GNi1j2) -- (GNi2j2);
\draw[activempmgrid] (GNi1j2) -- (GNi1j3);
\draw[activempmgrid] (GNi1j3) -- (GNi2j3);
\draw[activempmgrid] (GNi1j3) -- (GNi1j4);
\draw[activempmgrid] (GNi1j4) -- (GNi2j4);
\draw[activempmgrid] (GNi2j0) -- (GNi3j0);
\draw[activempmgrid] (GNi2j0) -- (GNi2j1);
\draw[activempmgrid] (GNi2j1) -- (GNi3j1);
\draw[activempmgrid] (GNi2j1) -- (GNi2j2);
\draw[activempmgrid] (GNi2j2) -- (GNi3j2);
\draw[activempmgrid] (GNi2j2) -- (GNi2j3);
\draw[activempmgrid] (GNi2j3) -- (GNi3j3);
\draw[activempmgrid] (GNi2j3) -- (GNi2j4);
\draw[activempmgrid] (GNi2j4) -- (GNi3j4);
\draw[activempmgrid] (GNi3j0) -- (GNi4j0);
\draw[activempmgrid] (GNi3j0) -- (GNi3j1);
\draw[activempmgrid] (GNi3j1) -- (GNi4j1);
\draw[activempmgrid] (GNi3j1) -- (GNi3j2);
\draw[activempmgrid] (GNi3j2) -- (GNi4j2);
\draw[activempmgrid] (GNi3j2) -- (GNi3j3);
\draw[activempmgrid] (GNi3j3) -- (GNi4j3);
\draw[activempmgrid] (GNi3j3) -- (GNi3j4);
\draw[activempmgrid] (GNi3j4) -- (GNi4j4);
\draw[activempmgrid] (GNi4j0) -- (GNi4j1);
\draw[activempmgrid] (GNi4j1) -- (GNi4j2);
\draw[activempmgrid] (GNi4j2) -- (GNi4j3);
\draw[activempmgrid] (GNi4j3) -- (GNi4j4);
\draw (GNi0j0) edge[thick,color=red,->] ($(GNi0j0) + (0.000000in,-0.006250in)$);
\draw (GNi0j1) edge[thick,color=red,->] ($(GNi0j1) + (0.000000in,-0.069625in)$);
\draw (GNi0j2) edge[thick,color=red,->] ($(GNi0j2) + (0.000000in,-0.090750in)$);
\draw (GNi0j3) edge[thick,color=red,->] ($(GNi0j3) + (0.000000in,-0.069625in)$);
\draw (GNi0j4) edge[thick,color=red,->] ($(GNi0j4) + (0.000000in,-0.006250in)$);
\draw (GNi1j0) edge[thick,color=red,->] ($(GNi1j0) + (0.073938in,-0.033062in)$);
\draw (GNi1j1) edge[thick,color=red,->] ($(GNi1j1) + (0.084500in,-0.096437in)$);
\draw (GNi1j2) edge[thick,color=red,->] ($(GNi1j2) + (0.095063in,-0.117563in)$);
\draw (GNi1j3) edge[thick,color=red,->] ($(GNi1j3) + (0.105625in,-0.096437in)$);
\draw (GNi1j4) edge[thick,color=red,->] ($(GNi1j4) + (0.116188in,-0.033062in)$);
\draw (GNi2j0) edge[thick,color=red,->] ($(GNi2j0) + (0.084500in,-0.081000in)$);
\draw (GNi2j1) edge[thick,color=red,->] ($(GNi2j1) + (0.105625in,-0.144375in)$);
\draw (GNi2j2) edge[thick,color=red,->] ($(GNi2j2) + (0.126750in,-0.165500in)$);
\draw (GNi2j3) edge[thick,color=red,->] ($(GNi2j3) + (0.147875in,-0.144375in)$);
\draw (GNi2j4) edge[thick,color=red,->] ($(GNi2j4) + (0.169000in,-0.081000in)$);
\draw (GNi3j0) edge[thick,color=red,->] ($(GNi3j0) + (0.031687in,-0.150063in)$);
\draw (GNi3j1) edge[thick,color=red,->] ($(GNi3j1) + (0.063375in,-0.213438in)$);
\draw (GNi3j2) edge[thick,color=red,->] ($(GNi3j2) + (0.095062in,-0.234563in)$);
\draw (GNi3j3) edge[thick,color=red,->] ($(GNi3j3) + (0.126750in,-0.213438in)$);
\draw (GNi3j4) edge[thick,color=red,->] ($(GNi3j4) + (0.158438in,-0.150063in)$);
\draw (GNi4j0) edge[thick,color=red,->] ($(GNi4j0) + (-0.084500in,-0.240250in)$);
\draw (GNi4j1) edge[thick,color=red,->] ($(GNi4j1) + (-0.042250in,-0.303625in)$);
\draw (GNi4j2) edge[thick,color=red,->] ($(GNi4j2) + (0.000000in,-0.324750in)$);
\draw (GNi4j3) edge[thick,color=red,->] ($(GNi4j3) + (0.042250in,-0.303625in)$);
\draw (GNi4j4) edge[thick,color=red,->] ($(GNi4j4) + (0.084500in,-0.240250in)$);
\node[activempmnode] (GNi0j0) at ($(0.000000in,-0.006250in) + (CS3)$) {};
\node[activempmnode] (GNi0j1) at ($(0.000000in,0.255375in) + (CS3)$) {};
\node[activempmnode] (GNi0j2) at ($(0.000000in,0.559250in) + (CS3)$) {};
\node[activempmnode] (GNi0j3) at ($(0.000000in,0.905375in) + (CS3)$) {};
\node[activempmnode] (GNi0j4) at ($(0.000000in,1.293750in) + (CS3)$) {};
\node[activempmnode] (GNi1j0) at ($(0.398938in,-0.033062in) + (CS3)$) {};
\node[activempmnode] (GNi1j1) at ($(0.409500in,0.228563in) + (CS3)$) {};
\node[activempmnode] (GNi1j2) at ($(0.420063in,0.532438in) + (CS3)$) {};
\node[activempmnode] (GNi1j3) at ($(0.430625in,0.878563in) + (CS3)$) {};
\node[activempmnode] (GNi1j4) at ($(0.441188in,1.266938in) + (CS3)$) {};
\node[activempmnode] (GNi2j0) at ($(0.734500in,-0.081000in) + (CS3)$) {};
\node[activempmnode] (GNi2j1) at ($(0.755625in,0.180625in) + (CS3)$) {};
\node[activempmnode] (GNi2j2) at ($(0.776750in,0.484500in) + (CS3)$) {};
\node[activempmnode] (GNi2j3) at ($(0.797875in,0.830625in) + (CS3)$) {};
\node[activempmnode] (GNi2j4) at ($(0.819000in,1.219000in) + (CS3)$) {};
\node[activempmnode] (GNi3j0) at ($(1.006687in,-0.150063in) + (CS3)$) {};
\node[activempmnode] (GNi3j1) at ($(1.038375in,0.111562in) + (CS3)$) {};
\node[activempmnode] (GNi3j2) at ($(1.070063in,0.415437in) + (CS3)$) {};
\node[activempmnode] (GNi3j3) at ($(1.101750in,0.761563in) + (CS3)$) {};
\node[activempmnode] (GNi3j4) at ($(1.133438in,1.149938in) + (CS3)$) {};
\node[activempmnode] (GNi4j0) at ($(1.215500in,-0.240250in) + (CS3)$) {};
\node[activempmnode] (GNi4j1) at ($(1.257750in,0.021375in) + (CS3)$) {};
\node[activempmnode] (GNi4j2) at ($(1.300000in,0.325250in) + (CS3)$) {};
\node[activempmnode] (GNi4j3) at ($(1.342250in,0.671375in) + (CS3)$) {};
\node[activempmnode] (GNi4j4) at ($(1.384500in,1.059750in) + (CS3)$) {};
\draw[activempmgrid] (GNi0j0) -- (GNi1j0);
\draw[activempmgrid] (GNi0j0) -- (GNi0j1);
\draw[activempmgrid] (GNi0j1) -- (GNi1j1);
\draw[activempmgrid] (GNi0j1) -- (GNi0j2);
\draw[activempmgrid] (GNi0j2) -- (GNi1j2);
\draw[activempmgrid] (GNi0j2) -- (GNi0j3);
\draw[activempmgrid] (GNi0j3) -- (GNi1j3);
\draw[activempmgrid] (GNi0j3) -- (GNi0j4);
\draw[activempmgrid] (GNi0j4) -- (GNi1j4);
\draw[activempmgrid] (GNi1j0) -- (GNi2j0);
\draw[activempmgrid] (GNi1j0) -- (GNi1j1);
\draw[activempmgrid] (GNi1j1) -- (GNi2j1);
\draw[activempmgrid] (GNi1j1) -- (GNi1j2);
\draw[activempmgrid] (GNi1j2) -- (GNi2j2);
\draw[activempmgrid] (GNi1j2) -- (GNi1j3);
\draw[activempmgrid] (GNi1j3) -- (GNi2j3);
\draw[activempmgrid] (GNi1j3) -- (GNi1j4);
\draw[activempmgrid] (GNi1j4) -- (GNi2j4);
\draw[activempmgrid] (GNi2j0) -- (GNi3j0);
\draw[activempmgrid] (GNi2j0) -- (GNi2j1);
\draw[activempmgrid] (GNi2j1) -- (GNi3j1);
\draw[activempmgrid] (GNi2j1) -- (GNi2j2);
\draw[activempmgrid] (GNi2j2) -- (GNi3j2);
\draw[activempmgrid] (GNi2j2) -- (GNi2j3);
\draw[activempmgrid] (GNi2j3) -- (GNi3j3);
\draw[activempmgrid] (GNi2j3) -- (GNi2j4);
\draw[activempmgrid] (GNi2j4) -- (GNi3j4);
\draw[activempmgrid] (GNi3j0) -- (GNi4j0);
\draw[activempmgrid] (GNi3j0) -- (GNi3j1);
\draw[activempmgrid] (GNi3j1) -- (GNi4j1);
\draw[activempmgrid] (GNi3j1) -- (GNi3j2);
\draw[activempmgrid] (GNi3j2) -- (GNi4j2);
\draw[activempmgrid] (GNi3j2) -- (GNi3j3);
\draw[activempmgrid] (GNi3j3) -- (GNi4j3);
\draw[activempmgrid] (GNi3j3) -- (GNi3j4);
\draw[activempmgrid] (GNi3j4) -- (GNi4j4);
\draw[activempmgrid] (GNi4j0) -- (GNi4j1);
\draw[activempmgrid] (GNi4j1) -- (GNi4j2);
\draw[activempmgrid] (GNi4j2) -- (GNi4j3);
\draw[activempmgrid] (GNi4j3) -- (GNi4j4);
\node[inactivempmnode] (GNi0j0) at ($(0.000000in,0.000000in) + (CS4)$) {};
\node[inactivempmnode] (GNi0j1) at ($(0.000000in,0.325000in) + (CS4)$) {};
\node[inactivempmnode] (GNi0j2) at ($(0.000000in,0.650000in) + (CS4)$) {};
\node[inactivempmnode] (GNi0j3) at ($(0.000000in,0.975000in) + (CS4)$) {};
\node[inactivempmnode] (GNi0j4) at ($(0.000000in,1.300000in) + (CS4)$) {};
\node[inactivempmnode] (GNi1j0) at ($(0.325000in,0.000000in) + (CS4)$) {};
\node[inactivempmnode] (GNi1j1) at ($(0.325000in,0.325000in) + (CS4)$) {};
\node[inactivempmnode] (GNi1j2) at ($(0.325000in,0.650000in) + (CS4)$) {};
\node[inactivempmnode] (GNi1j3) at ($(0.325000in,0.975000in) + (CS4)$) {};
\node[inactivempmnode] (GNi1j4) at ($(0.325000in,1.300000in) + (CS4)$) {};
\node[inactivempmnode] (GNi2j0) at ($(0.650000in,0.000000in) + (CS4)$) {};
\node[inactivempmnode] (GNi2j1) at ($(0.650000in,0.325000in) + (CS4)$) {};
\node[inactivempmnode] (GNi2j2) at ($(0.650000in,0.650000in) + (CS4)$) {};
\node[inactivempmnode] (GNi2j3) at ($(0.650000in,0.975000in) + (CS4)$) {};
\node[inactivempmnode] (GNi2j4) at ($(0.650000in,1.300000in) + (CS4)$) {};
\node[inactivempmnode] (GNi3j0) at ($(0.975000in,0.000000in) + (CS4)$) {};
\node[inactivempmnode] (GNi3j1) at ($(0.975000in,0.325000in) + (CS4)$) {};
\node[inactivempmnode] (GNi3j2) at ($(0.975000in,0.650000in) + (CS4)$) {};
\node[inactivempmnode] (GNi3j3) at ($(0.975000in,0.975000in) + (CS4)$) {};
\node[inactivempmnode] (GNi3j4) at ($(0.975000in,1.300000in) + (CS4)$) {};
\node[inactivempmnode] (GNi4j0) at ($(1.300000in,0.000000in) + (CS4)$) {};
\node[inactivempmnode] (GNi4j1) at ($(1.300000in,0.325000in) + (CS4)$) {};
\node[inactivempmnode] (GNi4j2) at ($(1.300000in,0.650000in) + (CS4)$) {};
\node[inactivempmnode] (GNi4j3) at ($(1.300000in,0.975000in) + (CS4)$) {};
\node[inactivempmnode] (GNi4j4) at ($(1.300000in,1.300000in) + (CS4)$) {};
\draw[inactivempmgrid] (GNi0j0) -- (GNi1j0);
\draw[inactivempmgrid] (GNi0j0) -- (GNi0j1);
\draw[inactivempmgrid] (GNi0j1) -- (GNi1j1);
\draw[inactivempmgrid] (GNi0j1) -- (GNi0j2);
\draw[inactivempmgrid] (GNi0j2) -- (GNi1j2);
\draw[inactivempmgrid] (GNi0j2) -- (GNi0j3);
\draw[inactivempmgrid] (GNi0j3) -- (GNi1j3);
\draw[inactivempmgrid] (GNi0j3) -- (GNi0j4);
\draw[inactivempmgrid] (GNi0j4) -- (GNi1j4);
\draw[inactivempmgrid] (GNi1j0) -- (GNi2j0);
\draw[inactivempmgrid] (GNi1j0) -- (GNi1j1);
\draw[inactivempmgrid] (GNi1j1) -- (GNi2j1);
\draw[inactivempmgrid] (GNi1j1) -- (GNi1j2);
\draw[inactivempmgrid] (GNi1j2) -- (GNi2j2);
\draw[inactivempmgrid] (GNi1j2) -- (GNi1j3);
\draw[inactivempmgrid] (GNi1j3) -- (GNi2j3);
\draw[inactivempmgrid] (GNi1j3) -- (GNi1j4);
\draw[inactivempmgrid] (GNi1j4) -- (GNi2j4);
\draw[inactivempmgrid] (GNi2j0) -- (GNi3j0);
\draw[inactivempmgrid] (GNi2j0) -- (GNi2j1);
\draw[inactivempmgrid] (GNi2j1) -- (GNi3j1);
\draw[inactivempmgrid] (GNi2j1) -- (GNi2j2);
\draw[inactivempmgrid] (GNi2j2) -- (GNi3j2);
\draw[inactivempmgrid] (GNi2j2) -- (GNi2j3);
\draw[inactivempmgrid] (GNi2j3) -- (GNi3j3);
\draw[inactivempmgrid] (GNi2j3) -- (GNi2j4);
\draw[inactivempmgrid] (GNi2j4) -- (GNi3j4);
\draw[inactivempmgrid] (GNi3j0) -- (GNi4j0);
\draw[inactivempmgrid] (GNi3j0) -- (GNi3j1);
\draw[inactivempmgrid] (GNi3j1) -- (GNi4j1);
\draw[inactivempmgrid] (GNi3j1) -- (GNi3j2);
\draw[inactivempmgrid] (GNi3j2) -- (GNi4j2);
\draw[inactivempmgrid] (GNi3j2) -- (GNi3j3);
\draw[inactivempmgrid] (GNi3j3) -- (GNi4j3);
\draw[inactivempmgrid] (GNi3j3) -- (GNi3j4);
\draw[inactivempmgrid] (GNi3j4) -- (GNi4j4);
\draw[inactivempmgrid] (GNi4j0) -- (GNi4j1);
\draw[inactivempmgrid] (GNi4j1) -- (GNi4j2);
\draw[inactivempmgrid] (GNi4j2) -- (GNi4j3);
\draw[inactivempmgrid] (GNi4j3) -- (GNi4j4);

